PDSum: Prototype-driven Continuous Summarization of Evolving Multi-document Sets Stream

Summarizing text-rich documents has been long studied in the literature, but most of the existing efforts have been made to summarize a static and predefined multi-document set. With the rapid development of online platforms for generating and distributing text-rich documents, there arises an urgent need for continuously summarizing dynamically evolving multi-document sets where the composition of documents and sets is changing over time. This is especially challenging as the summarization should be not only effective in incorporating relevant, novel, and distinctive information from each concurrent multi-document set, but also efficient in serving online applications. In this work, we propose a new summarization problem, Evolving Multi-Document sets stream Summarization (EMDS), and introduce a novel unsupervised algorithm PDSum with the idea of prototype-driven continuous summarization. PDSum builds a lightweight prototype of each multi-document set and exploits it to adapt to new documents while preserving accumulated knowledge from previous documents. To update new summaries, the most representative sentences for each multi-document set are extracted by measuring their similarities to the prototypes. A thorough evaluation with real multi-document sets streams demonstrates that PDSum outperforms state-of-the-art unsupervised multi-document summarization algorithms in EMDS in terms of relevance, novelty, and distinctiveness and is also robust to various evaluation settings.

==> Tables/Summary_WE2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\begin{tabular}{ccc}
\textbf{Date} & \textbf{Method} & \textbf{Summary} \\
 & Gold & Attackers in Bangladesh wielding machetes kill Nazimuddin Samad, a liberal blogger. \\
 & Summpip & The killing on wednesday, police said thursday. \\
 & Primera & Attackers in Bangladesh wielding machetes killed a liberal blogger, police said on Thursday, the latest in series of murders of secular activists by suspected Islamist militants. \\
\multirow{-4}{*}{4/7/2016} & PDSum & Men armed with machetes killed a secular activist at a crowded intersection in Dhaka, the Bangladeshi capital, a police official said on Thursday, the latest in a series of grisly attacks on intellectuals and bloggers who have written critically about militant Islam on social media. \\
 & Gold & Professor Rezaul Karim Siddique is killed in   the Bangladeshi city of Rajshahi in an ISIL attack. \\
 & Summpip & {\color[HTML]{70AD47} bangladesh professor was hacked to death a   university .} \\
 & Primera & In Bangladesh, men attacked and hacked to   death liberal blogger Nazimuddin Samad, 26, with machetes on Monday   night.Samad left his law classes at Jagganath University in \\
\multirow{-4}{*}{4/23/2016} & PDSum & A professor of English was hacked to death   and nearly beheaded near his home in northwestern Bangladesh on Saturday, in   what the police said they suspected was the latest in a series of targeted   killings by Islamist militants. \\
 & Gold & Xulhaz Mannan, a Bangladeshi employee of a   U.S. charity (USAID), who is also an editor for the country's only LGBT   magazine, and a friend are hacked to death in Dhaka, Bangladesh, by suspected   Islamist militants. Guards at the building were also injured. \\
 & Summpip & advertisement u.s. agency for international   development , police said . \\
 & Primera & Unidentified assailants fatally stabbed two   men in Bangladesh's capital Monday night, including a gay rights activist who   also worked for the U.S. Agency for International Development, police said \\
\multirow{-4}{*}{4/25/2016} & PDSum & Top   News  Gay rights activist killed in   Bangladesh  Posted  Islamist militants are suspected of hacking   to death a leading gay rights activist and a friend at an apartment in the   Bangladeshi capital of Dhaka.
\end{tabular}
\end{table}

==> Tables/performance_bak.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\centering
\small
%\setlength{\tabcolsep}{3pt}
\begin{tabular}{ccccccccc|cccccccc}
\cline{2-17}
 & \multicolumn{8}{c|}{WCEP} & \multicolumn{8}{c}{W2E} \\ \cline{2-17} 
 & R1 & R2 & RL & \multicolumn{1}{c|}{BS} & N-RL & \multicolumn{1}{c|}{N-BS} & D-RL & D-BS & R1 & R2 & RL & \multicolumn{1}{c|}{BS} & N-RL & \multicolumn{1}{c|}{N-BS} & D-RL & D-BS \\ \hline
DocCent & 20.06 & 5.20 & 16.02 & \multicolumn{1}{c|}{83.59} & 10.67 & \multicolumn{1}{c|}{79.77} & 99.96 & 31.99 & 16.06 & 3.88 & 13.06 & \multicolumn{1}{c|}{82.96} & 5.86 & \multicolumn{1}{c|}{78.65} & 98.65 & 19.92 \\
IncDocCent & 20.52 & 5.40 & 16.34 & \multicolumn{1}{c|}{83.73} & 10.51 & \multicolumn{1}{c|}{79.11} & 99.96 & 32.01 & 14.65 & 2.97 & 11.39 & \multicolumn{1}{c|}{82.73} & 5.16 & \multicolumn{1}{c|}{77.89} & \uline{98.71} & 19.67 \\
SentCent & 19.17 & 4.87 & 15.37 & \multicolumn{1}{c|}{83.38} & 10.30 & \multicolumn{1}{c|}{79.35} & {\ul 99.97} & 31.99 & 14.93 & 3.41 & 12.15 & \multicolumn{1}{c|}{82.78} &  5.91 & \multicolumn{1}{c|}{\textbf{79.24}} & 98.59 & 19.99 \\
IncSentCent & 19.64 & 4.99 & 15.64 & \multicolumn{1}{c|}{83.46} & 10.53 & \multicolumn{1}{c|}{79.24} & {\ul 99.97} & 31.99 & 14.94 & 3.39 & 12.19 & \multicolumn{1}{c|}{82.81} & 5.76 & \multicolumn{1}{c|}{ {\ul 79.19}} & 98.61 & 19.81 \\
Lexrank & 13.63 & 3.33 & 11.28 & \multicolumn{1}{c|}{82.01} & 9.11 & \multicolumn{1}{c|}{80.58} & {\ul 99.97} & 32.13 & 11.40 & 2.93 & 9.55 & \multicolumn{1}{c|}{81.24} & 5.12 & \multicolumn{1}{c|}{77.27} & \textbf{98.92} &  20.92 \\
Summpip & 21.72 &  7.04 & 17.28 & \multicolumn{1}{c|}{83.60} &  11.74 & \multicolumn{1}{c|}{81.21} & 99.95 & 32.03 & 16.12 & 4.83 & 12.76 & \multicolumn{1}{c|}{82.68} & 5.77 & \multicolumn{1}{c|}{78.39} & 97.70 & 20.44 \\
Primera & 20.87 & 6.84 & 18.45 & \multicolumn{1}{c|}{ 83.84} & 11.65 & \multicolumn{1}{c|}{80.70} & \textbf{99.99} &  32.14 &  16.28 & 5.69 &  14.24 & \multicolumn{1}{c|}{ 83.00} & 3.67 & \multicolumn{1}{c|}{75.61} & 95.38 & 19.25 \\ \hline
\textbf{PDSum} & \textbf{\begin{tabular}[c]{@{}c@{}}26.62\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.05}$\end{tabular}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}9.20\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.04}$\end{tabular}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}21.01\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.05}$\end{tabular}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}84.51\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}12.67\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.03}$\end{tabular}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\ul 81.27}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.04}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}99.95\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}32.23\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}19.61\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.10}$\end{tabular}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}6.48\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.06}$\end{tabular}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}15.75\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.09}$\end{tabular}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}83.26\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.02}$\end{tabular}\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}\uline{6.60}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.03}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}76.35\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.09}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\uline{98.71}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.02}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 21.45}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.03}$\end{tabular}\end{tabular} \\[-0.2em] \hline 

w/o doc-score & \begin{tabular}[c]{@{}c@{}}{\ul 26.44}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.07}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 9.13}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.04}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 20.85}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.06}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\ul 84.47}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}} {\ul 12.64} \\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.05}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{81.40}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.04}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}99.94\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{32.23}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 19.07}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 6.23}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.05}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 15.31}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.08}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\ul 83.20}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.02}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}6.56\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.03}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}76.60\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.08}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}98.68\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}21.41\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} \\[-0.2em]
w/o sent-score & \begin{tabular}[c]{@{}c@{}}22.75\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}7.42\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}17.81\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}83.60\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}11.27\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}80.47\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.03}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}99.94\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}32.04\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}14.22\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.02}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.02\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}11.38\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}81.26\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{7.37}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.27\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.07}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}98.08\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{22.67}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} \\[-0.2em]
w/o phrase-score & \begin{tabular}[c]{@{}c@{}}20.99\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.09}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.33\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.05}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}17.06\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.06}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}83.59\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.02}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}11.2\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.05}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}80.71\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.08}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}99.95\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.00}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\ul 32.21}\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.01}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}13.59\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.19}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.94\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.11}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}10.91\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.17}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}81.86\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.04}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}5.32\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.04}$\end{tabular}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}76.16\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.33}$\end{tabular}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}97.95\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.14}$\end{tabular}\end{tabular} & \begin{tabular}[c]{@{}c@{}}20.52\\[-0.5em] \begin{tabular}[c]{@{}c@{}}\scriptsize ${\pm 0.06}$\end{tabular}\end{tabular} \\[-0.2em] \hline
\end{tabular}
